SOLIDO: A Robust Watermarking Method for Speech Synthesis via Low-Rank Adaptation

The accelerated advancement of speech generative models has given rise to security issues, including model infringement and unauthorized abuse of content. Although existing generative watermarking techniques have proposed corresponding solutions, most methods require substantial computational overhead and training costs. In addition, some methods have limitations in robustness when handling variable-length inputs. To tackle these challenges, we propose \textsc{SOLIDO}, a novel generative watermarking method that integrates parameter-efficient fine-tuning with speech watermarking through low-rank adaptation (LoRA) for speech diffusion models. Concretely, the watermark encoder converts the watermark to align with the input of diffusion models. To achieve precise watermark extraction from variable-length inputs, the watermark decoder based on depthwise separable convolution is designed for watermark recovery. To further enhance speech generation performance and watermark extraction capability, we propose a speech-driven lightweight fine-tuning strategy, which reduces computational overhead through LoRA. Comprehensive experiments demonstrate that the proposed method ensures high-fidelity watermarked speech even at a large capacity of 2000 bps. Furthermore, against common individual and compound speech attacks, our SOLIDO achieves a maximum average extraction accuracy of 99.20\% and 98.43\%, respectively. It surpasses other state-of-the-art methods by nearly 23\% in resisting time-stretching attacks.

==> data.tex <==



%----ALgorithm-------------------------------------------------------
\newcommand{\lIfElse}[3]{\lIf{#1}{#2 \textbf{else}~#3}}
\begin{algorithm}[t]
\caption{Speech-Driven Low-Rank Adaption Fine-tuning Strategy.}
\label{algo}
\SetKwInOut{Require}{Require}
\SetKwInOut{Output}{Output}
% \SetKwRepeat{Repeat}{repeat}{until}

\Require{Training dataset $\mathcal{D}_{train}$, watermark $\mathbf{w}$, watermark embedder $\mathbf{Emb}(\cdot)$ and decoder $\mathbf{Dec}(\cdot)$ with their trainalbe parameters $W_{\mathbf{Emb}}$ and $W_{\math  bf{Dec}}$, trainalbe LoRA parameters $\Delta W$, diffusion model with frozen weights $\theta$, hyper-parameter $\alpha_t$, and diffusion step $T$.}


\Repeat{converged}{
$\mathbf{s}_0 \leftarrow \mathbf{s}_0 \sim \mathcal{D}_{train}$;

\tcp{Watermarking}
$\sigma = \mathbf{Emb}(\mathbf{w})$; \Comment $\mathbf{w} \in \{0, 1\}^l$

$\mathbf{s}_T \leftarrow \mathbf{s}_T \sim \mathcal{N}(0, \mathbf{I})$;

$\mathbf{x}_T \leftarrow \mathbf{x}_T = \mathbf{s}_T + \sigma$;
    
$\theta_{wm} \leftarrow \theta_{wm} = \theta + \Delta W$;

\tcp{Generating}
\For{$t \leftarrow T, ..., 1$}  
{
    \lIfElse{$t > 1$}{$\mathbf{z} \sim \mathcal{N}(0, \mathbf{I})$}{$\mathbf{z} \leftarrow 0$}
    
    $\mathbf{x}_{t-1} \leftarrow \frac{1}{\sqrt{\alpha_t}} \big(\mathbf{x}_{t-1} - \frac{1-\alpha_t}{\sqrt{1-\overline \alpha_t}} \mathbf{\epsilon}_{\theta_{wm}}(\mathbf{x}_{t-1}, t, c) \big) + \delta_t \mathbf z$\;
}

\Return $\mathbf{x}_0$;

\tcp{Extracting}
$\hat{\mathbf{w}} = \mathbf{Dec}(\mathbf{x}_0)$;

\tcp{Fine-tuning}
Take gradient descent step on:
$\nabla_{\Delta W + W_{\mathbf{Emb}} + W_{\mathbf{Dec}}}(|| \phi(\mathbf{s}_0), \phi(\mathbf{x}_0) ||_1) + || \log(\mathbf{STFT}(\mathbf{s}_0)), \log(\mathbf{STFT}(\mathbf{x}_0)) ||_1) - \sum_{i=1}^{k} w_i \log {\hat{w}_i} + (1-w_i) \log(1-\hat{w}_i)$;
}

\end{algorithm}

\begin{table*}[]
\centering  
\caption{Ablation Study of SpeakLoRA.}
\begin{tabular}{cccccccc}
\toprule
Rank & Alpha & STOI↑  & MOSL↑  & SSIM↑  & MCD↓   & ACC(\%)↑ & $\Delta$ACC(\%)  \\
\midrule
\rowcolor[HTML]{DDDDDD} 
4    & 16    & 0.9583 & 3.2147 & 0.9056 & 1.2888 & 98.93 & - \\
\midrule
4    & 4     & 0.9425 & 2.9048 & 0.8917 & 1.4885 & 98.17 & -0.76 \\
4    & 32    & 0.9548 & 3.0058 & 0.8986 & 1.4113 & 97.91 & -1.02 \\
8    & 8     & 0.9286 & 2.6133 & 0.8846 & 1.5756 & 97.29 & -1.71 \\ 
40   & 40    & 0.9444 & 2.8199 & 0.8892 & 1.5972 & 98.59 & -0.34 \\
80   & 80    & 0.9546 & 2.9849 & 0.8983 & 1.4471 & 98.36 & -0.57 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\renewcommand\arraystretch{0.5}
\setlength{\belowcaptionskip}{-0.01cm}
\caption{Fidelity of SpeakLoRA With Various Datasets in DiffWave. ↑/↓ indicates a higher/lower value is more desirable.}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{cccccccccc}
\toprule
 & \multicolumn{3}{c}{\textit{Generated $\leftrightarrow$ Natural}} & \multicolumn{3}{c}{\textit{Watermarked $\leftrightarrow$ Generated}} & \multicolumn{3}{c}{\textit{Watermarked $\leftrightarrow$ Natural}} \\
\cmidrule{2-10}
& LJSpeech    & LibriTTS   & \multicolumn{1}{c|}{LibriSpeech} & LJSpeech  & LibriTTS   & \multicolumn{1}{c|}{LibriSpeech}  & LJSpeech   & LibriTTS   & LibriSpeech   \\
\midrule
STOI↑   & 0.9655 & 0.9337 & \multicolumn{1}{c|}{0.9176} & 0.9583 & 0.9274 & \multicolumn{1}{c|}{0.9119} & 0.9618 & 0.9366 & 0.9189  \\
MOSL↑   & 3.5120 & 2.8156 & \multicolumn{1}{c|}{2.7788} & 3.2147 & 2.7180 & \multicolumn{1}{c|}{2.4667} & 3.4066 & 2.8153 & 2.4220  \\
SSIM↑   & 0.8453 & 0.8025 & \multicolumn{1}{c|}{0.6699} & 0.9056 & 0.8800 & \multicolumn{1}{c|}{0.8218}  & 0.8629 & 0.8395 & 0.7049  \\
MCD↓    & 6.2794 & 6.0407 & \multicolumn{1}{c|}{15.2482} & 1.2888 & 1.2626 & \multicolumn{1}{c|}{1.2243} & 5.9335 & 4.0157 & 14.7335 \\
ACC(\%)↑    & N/A    & N/A    & \multicolumn{1}{c|}{N/A}    & 98.93 & 98.33 & \multicolumn{1}{c|}{98.88}  & 98.93 & 98.33 & 99.02 \\
\bottomrule
\end{tabular}
}
\label{tab_fidelity}
\end{table*}

\begin{table*}[]
\centering
\caption{Capacity of SpeakLoRA.}
\begin{tabular}{cccccc}
\toprule
         & \multicolumn{5}{c}{Capacity (bps)} \\
         \cmidrule{2-6}
         & 100    & 500    & 1000   & 2000   & 5000     \\
         \midrule
STOI↑    & 0.9583 & 0.9520 & 0.9587 & 0.9022 & 0.8988 \\
MOSL↑    & 3.2147 & 3.0940 & 3.2137 & 2.5362 & 2.4832 \\
SSIM↑    & 0.9056 & 0.9022 & 0.9059 & 0.8686 & 0.8690 \\
MCD↓     & 1.2888 & 1.3125 & 1.3144 & 1.2931 & 1.3143 \\
ACC(\%)↑ & 98.93  & 93.14  & 94.35  & 81.31  & 82.39 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\caption{Specific settings and descriptions for each type of audio post-processing attack, \\ including the parameters and probabilities used in the audio attack simulator \\ and the parameters utilized for robustness experiment during evaluation.}
\setlength{\tabcolsep}{1mm}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{ccccl}
\toprule
Attack Type & Param. & Prob. & Param. (Infer)  & Description
\\
\midrule
\multicolumn{1}{l}{Non-Attack} &&&& \\
Non & - & 0.167 & - & Watermarked audio without attacking.   
\\
\midrule
\multicolumn{1}{l}{Distortion Attacks} &&&& \\
Low-Pass Filtering  & - & - & 3 kHz & Permiting watermark audio signals below the threshold to pass.
\\
Band-Pass Filtering & - & - & 0.3-8 kHz & Allowing watermark audio signals within the minimum and maximum thresholds to pass.                                          
\\
Echo & default & 0.167 & default & \multicolumn{1}{l}{Attenuating the watermarked audio volume by a factor of 0.4, delaying it by 100ms.} 
\\
Pink Noise & - & - & 0.5 & Adding pink background noise to the watermarked audio. 
\\
Gaussian Noise  & 15-20 dB & 0.167 & 5/10/15/20 dB & Adding white Gaussian noise to the watermarked audio.                         
\\
\midrule
\multicolumn{1}{l}{Desyn. Attacks} &&&& \\
Dither  & RPDF & 0.167 & TPDF & Applying eliminating nonlinear truncation distortion to the watermarked audio.  
\\
Cropping & 25\% (initial/final) & 0.167 & 50\% (initial/final) & Cropping initial and final of the watermarked audio based on cut-rate.
\\
Stretch & - & - & 0.5$\times$/2$\times$ & Stretching the time of the watermarked audio by a factor.
\\
Pitch Shift & 1/-1 & 0.167 & 2/-2 & Shifting the pitch of the watermarked audio by steps. 
\\
\bottomrule
\end{tabular}
}
\end{table*}

\begin{table*}[]
\centering
\caption{Robustness of proposed method against individual attacks.}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{ccccccccccccccccc}
\toprule
& & Lowpass & Bandpass & Echo & PN  & \multicolumn{4}{c}{GN} & \multicolumn{2}{c}{Cropping} & Dither & \multicolumn{2}{c}{Stretch} & \multicolumn{2}{c}{Pitch Shift}
\\
\cmidrule{2-17}
& & 3 kHz & 0.3-8 kHz & Default & 0.5 & 5 dB & 10 dB & 15 dB & 20 dB & Front & Behind & Default & 0.5$\times$ & 2$\times$  & 2 & -2         
\\
\midrule
\multirow{3}{*}{LJSpeech} & STOI & 0.9997 & 0.8612 & 0.7663 & 0.8443 & 0.8475 & 0.9115 & 0.9535 & 0.9777 & N/A  & N/A & 1.0000  & 1.0000 & 0.9999 & 0.7602 & 0.7924
\\
& MOSL↑ & 4.6185 & 3.7717 & 1.1702 & 1.0866 & 1.0372 & 1.0841 & 1.2235 & 1.5352 & N/A & N/A & 4.6439  & 4.6422 & 3.3034 & 1.0424 & 1.0445
\\
& ACC(\%)↑ & 98.51 & 98.89 & 97.25 & 98.18 & 98.34 & 98.66 & 98.85 & 98.90 & 96.57 & 94.73 & 98.81 & 98.76 & 98.84 & 71.10 & 73.61
\\
\midrule
\multirow{3}{*}{LibriTTS} & STOI & 0.9917 & 0.8604 & 0.7688 & 0.8139 & 0.8589 & 0.9154 & 0.9522 & 0.9735 & N/A  & N/A & 0.9920  & 0.9920 & 0.9919 & 0.7638 & 0.7848
\\
& MOSL↑ & 4.6140 & 3.5055 & 1.2534 & 1.1022 & 1.0756 & 1.1820 & 1.4297 & 1.8902 & N/A & N/A & 4.6438  & 4.6415 & 3.7832 & 1.0698 & 1.0705
\\
& ACC(\%)↑ & 97.48 & 98.03 & 96.85 & 96.48 & 97.77 & 98.33 & 98.49 & 98.49 & 91.26 & 97.49 & 98.33 & 98.33 & 98.43 & 70.28 & 68.45
\\
\midrule
\multirow{3}{*}{LibriSpeech} & STOI & 0.9957 & 0.8634 & 0.6294 & 0.8275 & 0.8918 & 0.9403 & 0.9697 & 0.9852 & N/A  & N/A & 0.9960  & 0.9960 & 0.9959 & 0.7723 & 0.7892
\\
& MOSL↑ & 4.6134 & 3.4651 & 1.1922 & 1.1411 & 1.1358 & 1.2973 & 1.5998 & 2.0498 & N/A & N/A & 4.6436  & 4.6432 & 4.1026 & 1.1087 & 1.1022
\\
& ACC(\%)↑ & 98.99 & 97.29 & 93.78 & 97.32 & 99.10 & 99.13 & 99.14 & 99.10 & 92.14 & 98.37 & 99.02 & 98.94 & 99.20 & 70.75 & 71.26
\\
\bottomrule
\end{tabular}
}
\end{table*}

\begin{table*}[]
\centering
\caption{Robustness of proposed method against compound attacks.}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
& & GN+BP  & GN+Echo & GN+Dither & GN+PN  & PN+BP  & PN+Echo & PN+Echo \\
\midrule
\multirow{3}{*}{LJSpeech} & STOI↑ & 0.8456 & 0.7490 & 0.9776 & 0.8406 & 0.7832 & 0.6558  & 0.8430  \\
& MOSL↑ & 1.4787 & 1.1105  & 1.5353 & 1.0721 & 1.2561 & 1.0465  & 1.0864  \\
& ACC(\%)↑  & 99.21   & 97.44  & 99.19 & 98.51 & 98.27 & 96.15  & 98.01  \\
\midrule
\multirow{3}{*}{LibriTTS} & STOI↑ & 0.8477 & 0.7520 & 0.9735 & 0.8098 & 0.7573 & 0.6351  & 0.8144  \\
& MOSL↑ & 1.7684 & 1.1612  & 1.8902 & 1.0889 & 1.2712 & 1.0547  & 1.1016  \\
& ACC(\%)↑  & 98.14   & 97.22  & 98.49 & 96.43 & 96.24 & 94.11  & 95.90  \\
\midrule
\multirow{3}{*}{LibriSpeech} & STOI↑ & 0.8545 & 0.6188 & 0.9852 & 0.8254 & 0.7584 & 0.5242  & 0.8280  \\
& MOSL↑ & 1.8520 & 1.1530  & 2.0498 & 1.1292 & 1.3383 & 1.0673  & 1.1444  \\
& ACC(\%)↑  & 97.57   & 94.24  & 99.10 & 97.22 & 95.46 & 89.87  & 97.33  \\
\bottomrule
\end{tabular}
}
\end{table*}


\begin{table*}[]
\centering
\caption{Comparison of Robustness with SOTA Methods against individual attacks. ↑ indicates a higher value is more desirable. \\ The best results are marked in \textbf{BOLD} and the second best results are \underline{underline}.}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{ccccccccccccccccc}
\toprule
\multirow{2}{*}{Attacks}  & \multirow{2}{*}{Param.}  & \multicolumn{3}{c}{AudioSeal~\cite{roman2024audioseal}} & \multicolumn{3}{c}{WavMark~\cite{chen2023wavmark}} & \multicolumn{3}{c}{TimbreWM~\cite{liu2024timebre}} & \multicolumn{3}{c}{TriniMark} & \multicolumn{3}{c}{SOLIDO(Ours)}   \\
\cmidrule{3-17}
&         & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC(\%)↑} & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC(\%)↑} & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC(\%)↑} & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC(\%)↑} & STOI↑  & MOSL↑  & ACC(\%)↑ \\
\midrule
Echo                         & Default & 0.7563 & 1.1845 & \multicolumn{1}{c|}{72.77}    & 0.6122 & 1.3716 & \multicolumn{1}{c|}{86.68}    & 0.7559 & 1.4720 & \multicolumn{1}{c|}{58.18}    & 0.7777 & 3.1347 & \multicolumn{1}{c|}{\underline{94.83}}    & \cellcolor[HTML]{DDDDDD}0.8612 & \cellcolor[HTML]{DDDDDD}3.7717 & \cellcolor[HTML]{DDDDDD}\textbf{98.89}    
\\
Pink                         & 0.5     & 0.9185 & 1.3537 & \multicolumn{1}{c|}{65.71}    & 0.8673 & 1.3019 & \multicolumn{1}{c|}{69.24}    & 0.8473 & 1.3773 & \multicolumn{1}{c|}{72.82}    & 0.8498 & 3.1282 & \multicolumn{1}{c|}{\underline{84.87}}    & \cellcolor[HTML]{DDDDDD}0.8443 & \cellcolor[HTML]{DDDDDD}1.0866 & \cellcolor[HTML]{DDDDDD}\textbf{98.18}    
\\
\multirow{3}{*}{Gaussian}    & 5 dB    & 0.8411 & 1.0415 & \multicolumn{1}{c|}{60.48}    & 0.8128 & 1.1016 & \multicolumn{1}{c|}{51.21}    & 0.8797 & 1.1871 & \multicolumn{1}{c|}{56.27}    & 0.8351 & 3.1257 & \multicolumn{1}{c|}{\underline{67.77}}    & \cellcolor[HTML]{DDDDDD}0.8475 & \cellcolor[HTML]{DDDDDD}1.0372 & \cellcolor[HTML]{DDDDDD}\textbf{98.34}    
\\
& 10 dB   & 0.9110 & 1.0995 & \multicolumn{1}{c|}{60.86}    & 0.8898 & 1.2217 & \multicolumn{1}{c|}{52.14}    & 0.9136 & 1.3347 & \multicolumn{1}{c|}{63.35}    & 0.9028 & 3.1320 & \multicolumn{1}{c|}{\underline{77.61}}    & \cellcolor[HTML]{DDDDDD}0.9115 & \cellcolor[HTML]{DDDDDD}1.0841 & \cellcolor[HTML]{DDDDDD}\textbf{98.66}    
\\
& 20 dB   & 0.9789 & 1.5987 & \multicolumn{1}{c|}{66.00}    & 0.9733 & 2.1236 & \multicolumn{1}{c|}{65.23}    & 0.9812 & 2.7424 & \multicolumn{1}{c|}{81.54}    & 0.9762 & 3.1270 & \multicolumn{1}{c|}{\underline{94.58}}    & \cellcolor[HTML]{DDDDDD}0.9777 & \cellcolor[HTML]{DDDDDD}1.5352 & \cellcolor[HTML]{DDDDDD}\textbf{98.90}    
\\
\multirow{2}{*}{Cropping}    & Front   & N/A    & N/A    & \multicolumn{1}{c|}{89.71}    & -      & -      & \multicolumn{1}{c|}{-}        & N/A    & N/A    & \multicolumn{1}{c|}{\textbf{99.3}4}    & -      & -      & \multicolumn{1}{c|}{-}        & \cellcolor[HTML]{DDDDDD}N/A    & \cellcolor[HTML]{DDDDDD}N/A    & \cellcolor[HTML]{DDDDDD}\underline{96.57}    
\\
& Behind  & N/A    & N/A    & \multicolumn{1}{c|}{64.60}    & -      & -      & \multicolumn{1}{c|}{-}        & N/A    & N/A    & \multicolumn{1}{c|}{\textbf{99.48}}    & -      & -      & \multicolumn{1}{c|}{-}        & \cellcolor[HTML]{DDDDDD}N/A    & \cellcolor[HTML]{DDDDDD}N/A    & \cellcolor[HTML]{DDDDDD}\underline{94.73}    
\\
\multirow{2}{*}{Pitch Shift} & 2       & 0.7848 & 1.0458 & \multicolumn{1}{c|}{\underline{59.57}}    & 0.7810 & 1.0475 & \multicolumn{1}{c|}{46.77}    & 0.7458 & 1.0390 & \multicolumn{1}{c|}{49.32}    & 0.7677 & 3.1250 & \multicolumn{1}{c|}{50.20}    & \cellcolor[HTML]{DDDDDD}0.7602 & \cellcolor[HTML]{DDDDDD}1.0424 & \cellcolor[HTML]{DDDDDD}\textbf{71.10}    
\\
& -2      & 0.7512 & 1.0435 & \multicolumn{1}{c|}{\underline{57.98}}    & 0.7958 & 1.0646 & \multicolumn{1}{c|}{43.94}    & 0.7817 & 1.0493 & \multicolumn{1}{c|}{49.35}    & 0.7957 & 3.1380 & \multicolumn{1}{c|}{50.06}    & \cellcolor[HTML]{DDDDDD}0.7924 & \cellcolor[HTML]{DDDDDD}1.0445 & \cellcolor[HTML]{DDDDDD}\textbf{73.61}      
\\
\bottomrule
\end{tabular}
}
\end{table*}


\begin{table*}
\setlength{\belowcaptionskip}{-0.01mm}
\centering
\caption{Comparison of Robustness against Compound Attacks with SOTA Methods.↑ indicates a higher value is more desirable. \\ The best results are marked in \textbf{BOLD} and the second best results are \underline{underline}.}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{ccccccccccccccccccc}
\toprule
 & \multicolumn{3}{c}{GN+BP} & \multicolumn{3}{c}{GN+Echo}  & \multicolumn{3}{c}{GN+PN} & \multicolumn{3}{c}{PN+BP} & \multicolumn{3}{c}{PN+Echo}  \\
 \cmidrule{2-16}
  & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC↑} & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC↑} & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC↑} & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC↑} & STOI↑  & MOSL↑  & ACC↑ \\
  \midrule
WavMark~\cite{chen2023wavmark}         & 0.8886 & 1.1139 & \multicolumn{1}{c|}{64.94}          & 0.5922 & 1.2798 & \multicolumn{1}{c|}{55.47}          & 0.8601 & 1.2292 & \multicolumn{1}{c|}{59.57}          & 0.8102 & 1.0785 & \multicolumn{1}{c|}{66.08}          & 0.5221 & 1.1868 & 56.17          \\
AudioSeal~\cite{roman2024audioseal}       & 0.8447 & 1.5308 & \multicolumn{1}{c|}{64.09}          & 0.7400 & 1.1177 & \multicolumn{1}{c|}{63.05}          & 0.9118 & 1.2292 & \multicolumn{1}{c|}{63.94}          & 0.8292 & 1.7364 & \multicolumn{1}{c|}{64.80}          & 0.7099 & 1.0912 & 62.80          \\
TimbreWM~\cite{liu2024timebre}        & 0.9853 & 4.0366 & \multicolumn{1}{c|}{79.71}          & 0.9853 & 4.0366 & \multicolumn{1}{c|}{74.58}          & 0.9853 & 4.0366 & \multicolumn{1}{c|}{67.64}          & 0.9853 & 4.0366 & \multicolumn{1}{c|}{70.85}          & 0.9853 & 4.0366 & 68.20          \\
TriniMark  & 0.8453 & 3.1356 & \multicolumn{1}{c|}{\underline{94.49}}    & 0.7555 & 3.1254 & \multicolumn{1}{c|}{\underline{90.71}}    & 0.8445 & 3.1340 & \multicolumn{1}{c|}{\underline{82.85}}    & 0.7853 & 3.1264 & \multicolumn{1}{c|}{\underline{85.24}}    & 0.6764 & 3.1323 & \underline{81.17}    \\
\rowcolor[HTML]{DDDDDD} 
SpeakLoRA(Ours) & 0.8497 & 2.1873 & \multicolumn{1}{c|}{\textbf{99.21}} & 0.7452 & 2.1925 & \multicolumn{1}{c|}{\textbf{97.44 }} & 0.9012 & 2.1896 & \multicolumn{1}{c|}{\textbf{98.51}} & 0.8194 & 2.1862 & \multicolumn{1}{c|}{\textbf{98.27}} & 0.6968 & 2.1907 & \textbf{96.15} \\
\bottomrule
\end{tabular}
}
\label{tab_robust_cmp_compo}
\end{table*}
Groot~\cite{liu2024groot}

% AudioSeal
% psn2 AVG STOI:0.7848, AVG MOSL:1.0458, AVG SSIM:0.5078, AVG MCD:4.1387, AVG ACC:0.5957
% psp2 AVG STOI:0.7512, AVG MOSL:1.0435, AVG SSIM:0.5063, AVG MCD:4.5309, AVG ACC:0.5798

% DeAR
% psn2 AVG STOI:0.6450, AVG MOSL:1.0491, AVG SSIM:0.4354, AVG MCD:33.4592, AVG ACC:0.7875
% psp2 AVG STOI:0.6265, AVG MOSL:1.0517, AVG SSIM:0.4383, AVG MCD:17.7168, AVG ACC:0.7306



\begin{table*}[]
\centering
\caption{Comparison of Robustness with SOTA Methods against individual attacks. ↑ indicates a higher value is more desirable. \\ The best results are marked in \textbf{BOLD} and the second best results are \underline{underline}.}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{ccccccccccccccccc}
\toprule
\multirow{2}{*}{Attacks}  & \multirow{2}{*}{Param.}  & \multicolumn{3}{c}{AudioSeal~\cite{roman2024audioseal}} & \multicolumn{3}{c}{WavMark~\cite{chen2023wavmark}} & \multicolumn{3}{c}{TimbreWM~\cite{liu2024timebre}} & \multicolumn{3}{c}{TriniMark} & \multicolumn{3}{c}{SOLIDO(Ours)}   \\
\cmidrule{3-17}
&         & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC(\%)↑} & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC(\%)↑} & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC(\%)↑} & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC(\%)↑} & STOI↑  & MOSL↑  & ACC(\%)↑ \\
\midrule
Echo                         & Default & 0.7563 & 1.1845 & \multicolumn{1}{c|}{72.77}    & 0.6122 & 1.3716 & \multicolumn{1}{c|}{86.68}    & 0.7559 & 1.4720 & \multicolumn{1}{c|}{58.18}    & 0.7777 & 3.1347 & \multicolumn{1}{c|}{\underline{94.83}}    & \cellcolor[HTML]{DDDDDD}0.8612 & \cellcolor[HTML]{DDDDDD}3.7717 & \cellcolor[HTML]{DDDDDD}\textbf{98.89}    
\\
Pink                         & 0.5     & 0.9185 & 1.3537 & \multicolumn{1}{c|}{65.71}    & 0.8673 & 1.3019 & \multicolumn{1}{c|}{69.24}    & 0.8473 & 1.3773 & \multicolumn{1}{c|}{72.82}    & 0.8498 & 3.1282 & \multicolumn{1}{c|}{\underline{84.87}}    & \cellcolor[HTML]{DDDDDD}0.8443 & \cellcolor[HTML]{DDDDDD}1.0866 & \cellcolor[HTML]{DDDDDD}\textbf{98.18}    
\\
\multirow{3}{*}{Gaussian}    & 5 dB    & 0.8411 & 1.0415 & \multicolumn{1}{c|}{60.48}    & 0.8128 & 1.1016 & \multicolumn{1}{c|}{51.21}    & 0.8797 & 1.1871 & \multicolumn{1}{c|}{56.27}    & 0.8351 & 3.1257 & \multicolumn{1}{c|}{\underline{67.77}}    & \cellcolor[HTML]{DDDDDD}0.8475 & \cellcolor[HTML]{DDDDDD}1.0372 & \cellcolor[HTML]{DDDDDD}\textbf{98.34}    
\\
& 10 dB   & 0.9110 & 1.0995 & \multicolumn{1}{c|}{60.86}    & 0.8898 & 1.2217 & \multicolumn{1}{c|}{52.14}    & 0.9136 & 1.3347 & \multicolumn{1}{c|}{63.35}    & 0.9028 & 3.1320 & \multicolumn{1}{c|}{\underline{77.61}}    & \cellcolor[HTML]{DDDDDD}0.9115 & \cellcolor[HTML]{DDDDDD}1.0841 & \cellcolor[HTML]{DDDDDD}\textbf{98.66}    
\\
& 20 dB   & 0.9789 & 1.5987 & \multicolumn{1}{c|}{66.00}    & 0.9733 & 2.1236 & \multicolumn{1}{c|}{65.23}    & 0.9812 & 2.7424 & \multicolumn{1}{c|}{81.54}    & 0.9762 & 3.1270 & \multicolumn{1}{c|}{\underline{94.58}}    & \cellcolor[HTML]{DDDDDD}0.9777 & \cellcolor[HTML]{DDDDDD}1.5352 & \cellcolor[HTML]{DDDDDD}\textbf{98.90}    
\\
\multirow{2}{*}{Cropping}    & Front   & N/A    & N/A    & \multicolumn{1}{c|}{89.71}    & -      & -      & \multicolumn{1}{c|}{-}        & N/A    & N/A    & \multicolumn{1}{c|}{\textbf{99.3}4}    & -      & -      & \multicolumn{1}{c|}{-}        & \cellcolor[HTML]{DDDDDD}N/A    & \cellcolor[HTML]{DDDDDD}N/A    & \cellcolor[HTML]{DDDDDD}\underline{96.57}    
\\
& Behind  & N/A    & N/A    & \multicolumn{1}{c|}{64.60}    & -      & -      & \multicolumn{1}{c|}{-}        & N/A    & N/A    & \multicolumn{1}{c|}{\textbf{99.48}}    & -      & -      & \multicolumn{1}{c|}{-}        & \cellcolor[HTML]{DDDDDD}N/A    & \cellcolor[HTML]{DDDDDD}N/A    & \cellcolor[HTML]{DDDDDD}\underline{94.73}    
\\
\multirow{2}{*}{Pitch Shift} & 2       & 0.7848 & 1.0458 & \multicolumn{1}{c|}{\underline{59.57}}    & 0.7810 & 1.0475 & \multicolumn{1}{c|}{46.77}    & 0.7458 & 1.0390 & \multicolumn{1}{c|}{49.32}    & 0.7677 & 3.1250 & \multicolumn{1}{c|}{50.20}    & \cellcolor[HTML]{DDDDDD}0.7602 & \cellcolor[HTML]{DDDDDD}1.0424 & \cellcolor[HTML]{DDDDDD}\textbf{71.10}    
\\
& -2      & 0.7512 & 1.0435 & \multicolumn{1}{c|}{\underline{57.98}}    & 0.7958 & 1.0646 & \multicolumn{1}{c|}{43.94}    & 0.7817 & 1.0493 & \multicolumn{1}{c|}{49.35}    & 0.7957 & 3.1380 & \multicolumn{1}{c|}{50.06}    & \cellcolor[HTML]{DDDDDD}0.7924 & \cellcolor[HTML]{DDDDDD}1.0445 & \cellcolor[HTML]{DDDDDD}\textbf{73.61}      
\\
\bottomrule
\end{tabular}
}
\end{table*}

\begin{table*}
\setlength{\belowcaptionskip}{-0.01mm}
\centering
\caption{Comparison of Robustness against Compound Attacks with SOTA Methods.↑ indicates a higher value is more desirable. \\ The best results are marked in \textbf{BOLD} and the second best results are \underline{underline}.}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{ccccccccccccccccccc}
\toprule
 & \multicolumn{3}{c}{GN+BP} & \multicolumn{3}{c}{GN+Echo}  & \multicolumn{3}{c}{GN+PN} & \multicolumn{3}{c}{PN+BP} & \multicolumn{3}{c}{PN+Echo}  \\
 \cmidrule{2-16}
  & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC↑} & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC↑} & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC↑} & STOI↑  & MOSL↑  & \multicolumn{1}{c|}{ACC↑} & STOI↑  & MOSL↑  & ACC↑ \\
  \midrule
WavMark~\cite{chen2023wavmark}         & 0.8886 & 1.1139 & \multicolumn{1}{c|}{64.94}          & 0.5922 & 1.2798 & \multicolumn{1}{c|}{55.47}          & 0.8601 & 1.2292 & \multicolumn{1}{c|}{59.57}          & 0.8102 & 1.0785 & \multicolumn{1}{c|}{66.08}          & 0.5221 & 1.1868 & 56.17          \\
AudioSeal~\cite{roman2024audioseal}       & 0.8447 & 1.5308 & \multicolumn{1}{c|}{64.09}          & 0.7400 & 1.1177 & \multicolumn{1}{c|}{63.05}          & 0.9118 & 1.2292 & \multicolumn{1}{c|}{63.94}          & 0.8292 & 1.7364 & \multicolumn{1}{c|}{64.80}          & 0.7099 & 1.0912 & 62.80          \\
TimbreWM~\cite{liu2024timebre}        & 0.9853 & 4.0366 & \multicolumn{1}{c|}{79.71}          & 0.9853 & 4.0366 & \multicolumn{1}{c|}{74.58}          & 0.9853 & 4.0366 & \multicolumn{1}{c|}{67.64}          & 0.9853 & 4.0366 & \multicolumn{1}{c|}{70.85}          & 0.9853 & 4.0366 & 68.20          \\
TriniMark  & 0.8453 & 3.1356 & \multicolumn{1}{c|}{\underline{94.49}}    & 0.7555 & 3.1254 & \multicolumn{1}{c|}{\underline{90.71}}    & 0.8445 & 3.1340 & \multicolumn{1}{c|}{\underline{82.85}}    & 0.7853 & 3.1264 & \multicolumn{1}{c|}{\underline{85.24}}    & 0.6764 & 3.1323 & \underline{81.17}    \\
\rowcolor[HTML]{DDDDDD} 
SOLIDO(Ours) & 0.8497 & 2.1873 & \multicolumn{1}{c|}{\textbf{99.21}} & 0.7452 & 2.1925 & \multicolumn{1}{c|}{\textbf{97.44 }} & 0.9012 & 2.1896 & \multicolumn{1}{c|}{\textbf{98.51}} & 0.8194 & 2.1862 & \multicolumn{1}{c|}{\textbf{98.27}} & 0.6968 & 2.1907 & \textbf{96.15} \\
\bottomrule
\end{tabular}
}
\label{tab_robust_cmp_compo}
\end{table*}

